Self-Binarizing Networks

We present a method to train self-binarizing neural networks, that is, networks that evolve their weights and activations during training to become binary. To obtain similar binary networks, existing methods rely on the sign activation function. This function, however, has no gradients for non-zero values, which makes standard backpropagation impossible. To circumvent the difficulty of training a network relying on the sign activation function, these methods alternate between floating-point and binary representations of the network during training, which is sub-optimal and inefficient. We approach the binarization task by training on a unique representation involving a smooth activation function, which is iteratively sharpened during training until it becomes a binary representation equivalent to the sign activation function. Additionally, we introduce a new technique to perform binary batch normalization that simplifies the conventional batch normalization by transforming it into a simple comparison operation. This is unlike existing methods, which are forced to the retain the conventional floating-point-based batch normalization. Our binary networks, apart from displaying advantages of lower memory and computation as compared to conventional floating-point and binary networks, also show higher classification accuracy than existing state-of-the-art methods on multiple benchmark datasets.

==> 20_RelatedWork.tex <==
%%%%%%%%%%%%%%%%%%
%% RELATED WORK %%
%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:two}
Making deep networks memory and computation efficient has been approached in various ways.
In this section we cover the some of the relevant literature and explain how our work is positioned with respect to the state-of-the-art. The interested reader may refer to~\citet{cheng_survey_2018}, \citet{ota_survey_2017}, and~\citet{wang_survey_2018} for a wider coverage.

\subsection{Efficient convolutions}
\citet{howard2017mobilenets,zhang2017shufflenet,freeman2018effnet} employ variations of convolutional layers by taking advantage of the separability of the kernels either by convolving with a group of input channels or by splitting the kernels across the dimensions. In addition to depth-wise convolutions, MobileNetV2~\citep{sandler2018inverted} uses inverted residual structures to learn how to combine the inputs in a residual block. In general, these methods try to design a model that computes convolutions in an efficient manner. This is different from this work because it focuses on redesigning the structure of the network, while ours tries to reduce the memory requirements by using lower precision parameters. However, our method can be applied to these networks as well.

\subsection{Compression and pruning}
Due to the redundancy in deep neural networks~\citep{cheng2015exploration}, there are some weights that contribute more to the output than others. The process of removing the less contributing weights is called pruning. In~\citet{lecun1990optimal}, a weight's contribution is measured by the effect on the training error when this parameter is zeroed. In Deep Compression, the weights with lowest absolute value are pruned and the remaining are quantized and compressed using Huffman coding~\citep{han2015deep}. In other work, Fisher Information is used to measure the amount of information the output carries about each parameter~\citep{tu2016ranking}. 

While these approaches often operate on already trained networks and fine-tune them after compression, our method trains a network to a binary state from scratch without removing any parameters or feature maps. This allows us to retain the original structure of the network, while still leaving the potential for further compression after or during binarization using pruning techniques.

\subsection{Quantization}
Quantized neural networks~\citep{hubara2016quantized,zhou2016dorefa,zhou2017incremental} occupy less memory while retaining similar performance as their full precision counterparts. DoReFaNet~\citep{zhou2016dorefa} proposes to train low bitwidth networks with low bitwidth gradients using stochastic quantization. Similarly,~\citet{zhou2017incremental} devise a weight partitioning technique to incrementally quantize the network at each step.

The degree of quantization can vary between techniques. ~\citet{deng2018gxnor},~\citet{zhu2016trained}, and~\citet{fengfu2016ternary} quantize weights to three levels, i.e two bits only. These quantizations, while severe, still allow for accurate inference. However, specialized hardware is needed to take advantage of the underlying ternary operations. These works are quite similar in philosophy to our method, but we will be only deal with the extreme scenario of binary i.e a single bit quantization.

\subsection{Binarization and Gradient estimation}
Expectation BackPropagation (EBP) paved the way for training neural networks for precision limited-hardware~\citep{soudry2014expectation}. BinaryConnect~\citep{courbariaux2015binaryconnect} extends the idea to train neural networks with binary weights. The authors later propose BinaryNet~\citep{courbariaux2016binarized} to binarize activations as well. Similarly, XNORNet~\citep{rastegari2016xnor} extends BinaryNet by adding a scaling factor to the parameters of every layer while keeping the weights and activations binary. ABCNet~\citep{lin2017towards} approximates full precision parameters as a linear combination of binary weights and uses multiple binary activations to compensate for the information loss arising from quantization. \citet{hou2016loss} use Hessian approximations to minimize loss with respect to the binary weights during training.

In all these binarization methods, the binarization process is non-differentiable leading to approximations during the training that can affect the final accuracy. In contrast, we use a differentiable function to progressively binarize the network and improves its accuracy. Additionally, we differ from these techniques as we remove all floating point operations at inference time, by properly converting the batch normalization to a boolean operation.

